A Novel ILP Framework for Summarizing Content with High Lexical Variety

Summarizing content contributed by individuals can be challenging, because people make different lexical choices even when describing the same events. However, there remains a significant need to summarize such content. Examples include the student responses to post-class reflective questions, product reviews, and news articles published by different news agencies related to the same events. High lexical diversity of these documents hinders the system's ability to effectively identify salient content and reduce summary redundancy. In this paper, we overcome this issue by introducing an integer linear programming-based summarization framework. It incorporates a low-rank approximation to the sentence-word co-occurrence matrix to intrinsically group semantically-similar lexical items. We conduct extensive experiments on datasets of student responses, product reviews, and news documents. Our approach compares favorably to a number of extractive baselines as well as a neural abstractive summarization system. The paper finally sheds light on when and why the proposed framework is effective at summarizing content with high lexical variety.

==> table_extrinsic_rouge_cutoff.tex <==
\begin{small}
\begin{tabular}{l l | lll| lll |c}
\hline\hline
 &  & \multicolumn{3}{c|}{\textbf{R-1}} & \multicolumn{3}{c|}{\textbf{R-2}} & \textbf{Human}\\ 
 & \multicolumn{1}{l|}{\textbf{System}} & \ \ R & \ \ P  & \ \ F & \ \ R & \ \ P  & \ \ F & \textbf{Preference}\\
\hline
Eng  &  MEAD  &  .192$^*$  &  .179$^*$  &  .161$^*$  &  .052$^*$  &  .054$^*$  &  .046$^*$ & -\\
  &  LexRank  &  .303$^*$  &  .286$^*$  &  .262$^*$  &  .093  &  .097  &  .087 & -\\
  &  SumBasic  &  .387  &  \bf.337  &  \bf.323  &  .090$^*$  &  .089$^*$  &  .082$^*$ & 26.9\%\\
  &  ILP  &  .364$^*$  &  .329  &  .308  &  .123  &  .124  &  .110  &  24.1\% \\
  &  ILP+MC  &  \bf\underline{.392}  &  \underline{.335}  &  \underline{.322}  &  \bf\underline{.130}  &  \bf\underline{.127}  &  \bf\underline{.114}  &  \bf\underline{29.4\%} \\\hline  
Stat2015  &  MEAD  &  .225$^*$  &  .217$^*$  &  .213$^*$  &  .073$^*$  &  .073$^*$  &  .071$^*$ & -\\
  &  LexRank  &  .334$^*$  &  .346  &  .325$^*$  &  .154  &  .147  &  .142 & -\\
  &  SumBasic  &  \bf.457$^*$  &  \bf.424$^*$  &  \bf.427$^*$  &  \bf.193  &  .169  &  \bf.174 & \bf 30.7\%\\
   &  ILP  &  .405  &  .396  &  .390  &  .186  &  \bf.175  &  \bf.174  & \ 29.2\%$^*$ \\
   &  ILP+MC  &  .401  &  .372  &  .375  &  .183  &  .164  &  .167  &  \underline{29.6\%} \\\hline
Stat2016  &  MEAD  &  .364$^*$  &  .419$^*$  &  .378$^*$  &  .172$^*$  &  .213  &  .181 & -\\
  &  LexRank  &  .397$^*$  &  .431  &  .407$^*$  &  .191  &  .209  &  .195 & -\\
  &  SumBasic  &  \bf.554$^*$  &  \bf.569$^*$  &  \bf.557$^*$  &  \bf.295$^*$  &  \bf.298$^*$  &  \bf.294$^*$ & \bf 32.9\%\\
    &  ILP  &  .482  &  .516  &  .496  &  .262$^*$   &  .283$^*$  &  .270$^*$  & 29.1\% \\
    &  ILP+MC  &  .457  &  .489  &  .465  &  .214 &  .230  &  .218  & 28.0\% \\\hline
CS2016  &  MEAD  &  .221$^*$  &  .190$^*$  &  .195$^*$  &  .056$^*$  &  .050$^*$  &  .050$^*$ & -\\
  &  LexRank  &  .285$^*$  &  .296$^*$  &  .282$^*$  &  .085$^*$  &  .089$^*$  &  .084$^*$ & -\\
  &  SumBasic  &  \bf.408  &  .408  &  \bf.398  &  .141  &  .144  &  .139 & 31.5\%\\
  &  ILP  &  .374  &  .408  &  .382  &  .141  &  .155  &  .144 & \ 24.4\%$^*$ \\
   &  ILP+MC  &  \underline{.398}  &  \bf\underline{.409}  &  \underline{.395}  &  \bf\underline{.154}  &  \bf\underline{.156}  &  \bf\underline{.151}  & \bf\underline{32.7\%} \\\hline
camera  &  MEAD  &  \bf.475  &  \bf.478  &  \bf.474  &  \bf.207  &  \bf.217  &  \bf.211 & -\\
  &  LexRank  &  .439  &  .456  &  .446  &  .181  &  .188  &  .184 & -\\
  &  SumBasic  &  \bf.475  &  .472  &  .473  &  .168  &  .166$^*$  &  .167 & \ 23.9\%$^*$\\
  &  ILP  &  .457  &  .466  &  .460  &  .165  &  .165  &  .165  & \bf36.9\% \\
   &  ILP+MC  &  .447  &  .449  &  .447  &  .157  &  .158  &  .157  & 32.5\% \\\hline
movie  &  MEAD  &  .394  &  .408  &  .398  &  .131  &  .136  &  .132 & -\\
  &  LexRank  &  .434$^*$  &  .428  &  .417  &  \bf.147  &  \bf.141  &  \bf.139 & -\\
  &  SumBasic  &  \bf.441  &  \bf.437  &  \bf.437  &  .098  &  .097  &  .097 & \ 27.6\%$^*$\\
   &  ILP  &  .435  &  .424  &  .427  &  .091$^*$  &  .087$^*$  &  .088$^*$  & \bf38.2\% \\
   &  ILP+MC  &  \underline{.436}  &  \underline{.427}  &  \underline{.429}  &  \underline{.106}  &  \underline{.100}  &  \underline{.102}  & 21.8\% \\\hline
peer  &  MEAD  &  .469  &  .494  &  .479  &  .242  &  .255  &  .248 & -\\
  &  LexRank  &  .444  &  .461  &  .451  &  .196  &  .214  &  .204 & -\\
  &  SumBasic  &  .473  &  .470  &  .471  &  .154$^*$  &  .149  &  .151 & 23.3\%\\
  &  ILP  &  .466  &  .469  &  .466  &  .199  &  .196  &  .197  & \bf34.4\% \\
 &  ILP+MC  &  \bf\underline{.491}  &  \bf\underline{.496}  &  \bf\underline{.492}  &  \bf\underline{.261}  &  \bf\underline{.262}  &  \bf\underline{.260}  & 22.2\% \\\hline
DUC04  &  MEAD  &  .352  &  .354  &  .351  &  .076  &  .076  &  .076 & -\\
  &  LexRank  &  .354  &  .364  &  .358  &  .076  &  .078  &  .077 & -\\
  &  SumBasic  &  .364$^*$  &  .365  &  .365$^*$  &  .066  &  .066  &  .066 & \ 24.9\%$^*$\\
  &   ILP  &  \bf.377$^*$  &  \bf.381$^*$  &  \bf.379$^*$  &  \bf.092$^*$  &  \bf.093$^*$  &  \bf.092$^*$  & \ 27.3\%$^*$ \\
  &    ILP+MC  &  .342  &  .351  &  .346  &  .072  &  .074  &  .072  &\bf\underline{31.1\%}\\
  & Best DUC & .418 & - & - & .107 & - & - & - \\\hline
 \hline
\end{tabular}
\end{small}





==> table_synthesize_res.tex <==
\begin{footnotesize}
\begin{tabular}{l|l| l| lll | lll}
\hline\hline 
 &  &  & \multicolumn{3}{c|}{\textbf{ROUGE$^-$1}} & \multicolumn{3}{c}{\textbf{ROUGE$^-$2}} \\ 
 & $\alpha_{b=1}$ & \multicolumn{1}{l|}{\textbf{System}} & R & P  & F & R & P & F \\
\hline
  
%  &  16.0  &  ILP  &  .320  &  .307  &  .280  &  .097  &  .107  &  .092  &  .112  &  .110  &  .076 \\
%  &    &  ILP+MC  &  \bf{.352$^+$}  &  \bf{.309}  &  \bf{.293}  &  .095  &  .103  &  .088  &  \bf{.128$^+$}  &  \bf{.115}  &  \bf{.082} \\
  &  26.5  &  ILP  &  .341  &  .318  &  .295  &  .112  &  .114  &  .102   \\
  &    &  ILP+MC  &  \bf{.378$^+$}  &  \bf{.324}  &  \bf{.311}  &  .112  &  .114  &  .100  \\
Eng  &  34.1  &  ILP  &  .364  &  .329  &  .308  &  .123  &  .124  &  .110   \\
  &    &  ILP+MC  &  \bf{.392$^+$}  &  \bf{.335}  &  \bf{.322}  &  \bf{.130}  &  \bf{.127}  &  \bf{.114}  \\
  &  36.0  &  ILP  &  .358  &  .327  &  .306  &  .119  &  .120  &  .107 \\
  &    &  ILP+MC  &  \bf{.397$^+$}  &  \bf{.339}  &  \bf{.327}  &  \bf{.126}  &  \bf{.123}  &  \bf{.111}   \\
%  &  38.6  &  ILP  &  .334  &  .308  &  .285  &  .099  &  .097  &  .087  &  .115  &  .100  &  .073 \\
%  &    &  ILP+MC  &  \bf{.369}  &  \bf{.324}  &  \bf{.307}  &  \bf{.106}  &  \bf{.105}  &  \bf{.094}  &  \bf{.133}  &  \bf{.120$^+$}  &  \bf{.084} \\
\hline
  &  11.9  &  ILP  &  .401  &  .395  &  .387  &  .183  &  .173  &  .172  \\
  &    &  ILP+MC  &  .362$^-$  &  .340$^-$  &  .341$^-$  &  .161  &  .149$^-$  &  .149$^-$ \\
Stat2015  &  18.1  &  ILP  &  .405  &  .396  &  .390  &  .186  &  .175  &  .174  \\
  &    &  ILP+MC  &  .401  &  .372  &  .375  &  .183  &  .164  &  .167   \\
  &  21.0  &  ILP  &  .394  &  .391  &  .382  &  .172  &  .161  &  .160  \\
  &    &  ILP+MC  &  .372  &  .352$^-$  &  .352  &  .156  &  .147  &  .147   \\
\hline  
%  &  5.4  &  ILP  &  .461  &  .496  &  .475  &  .243  &  .263  &  .251  &  .195  &  .229  &  .205 \\
%  &    &  ILP+MC  &  \bf{.468}  &  .489  &  .475  &  .218  &  .225$^-$  &  .220  &  \bf{.202}  &  .224  &  \bf{.207} \\
  &  13.2  &  ILP  &  .467  &  .500  &  .480  &  .252  &  .271  &  .259   \\
  &    &  ILP+MC  &  .463  &  .486  &  .471  &  .212$^-$  &  .222$^-$  &  .215$^-$  \\
Stat2016  &  20.9  &  ILP  &  .482  &  .516  &  .496  &  .262  &  .283  &  .270  \\
  &    &  ILP+MC  &  .457  &  .489  &  .465  &  .214$^-$  &  .230$^-$  &  .218$^-$  \\
  &  23.7  &  ILP  &  .455  &  .488  &  .468  &  .244  &  .265  &  .252  \\
  &    &  ILP+MC  &  \bf{.462}  &  .480  &  .467  &  .213  &  .220$^-$  &  .214$^-$   \\
%  &  29.9  &  ILP  &  .421  &  .451  &  .432  &  .193  &  .209  &  .199  &  .169  &  .196  &  .176 \\
%  &    &  ILP+MC  &  .384  &  .400$^-$  &  .389$^-$  &  .143$^-$  &  .151$^-$  &  .146$^-$  &  .142$^-$  &  .156$^-$  &  .145$^-$ \\
\hline

  &  11.0  &  ILP  &  .362  &  .395  &  .369  &  .138  &  .150  &  .140   \\
  &    &  ILP+MC  &  \bf{.386}  &  .395  &  \bf{.382}  &  .138  &  .140  &  .135   \\
%  &  19.3  &  ILP  &  .362  &  .393  &  .368  &  .139  &  .151  &  .141  &  .136  &  .164  &  .136 \\
%  &    &  ILP+MC  &  \bf{.405$^+$}  &  \bf{.416}  &  \bf{.402$^+$}  &  \bf{.156$^+$}  &  \bf{.159}  &  \bf{.154}  &  \bf{.165$^+$}  &  \bf{.176}  &  \bf{.157$^+$} \\
CS  &  25.6  &  ILP  &  .374  &  .408  &  .382  &  .141  &  .155  &  .144  \\
  &    &  ILP+MC  &  \bf{.398}  &  \bf{.409}  &  \bf{.395}  &  \bf{.154}  &  \bf{.156}  &  \bf{.151}   \\
  %&  28.0  &  ILP  &  .354  &  .386  &  .361  &  .133  &  .144  &  .135  &  .127  &  .157  &  .129 \\
  %&    &  ILP+MC  &  \bf{.360}  &  .386  &  .361  &  \bf{.135}  &  \bf{.146}  &  .133  &  \bf{.136}  &  \bf{.163}  &  \bf{.130} \\
  &  34.2  &  ILP  &  .296  &  .330  &  .306  &  .091  &  .108  &  .097   \\
  &    &  ILP+MC  &  \bf{.335$^+$}  &  \bf{.347}  &  \bf{.334}  &  \bf{.102}  &  .106  &  \bf{.102}   \\
\hline
   &  78.7  &  ILP  &  .453  &  .460  &  .456  &  .166  &  .166  &  .166   \\
  &    &  ILP+MC  &  .418  &  .430  &  .423  &  .137  &  .142  &  .139  \\
camera  &  84.9  &  ILP  &  .457  &  .466  &  .460  &  .165  &  .165  &  .165  \\
  &    &  ILP+MC  &  .447  &  .449  &  .447  &  .157  &  .158  &  .157   \\
  &  85.8  &  ILP  &  .452  &  .465  &  .457  &  .156  &  .159  &  .158  \\
  &    &  ILP+MC  &  \bf{.458}  &  \bf{.469}  &  \bf{.462}  &  \bf{.166}  &  \bf{.170}  &  \bf{.168}  \\
  \hline
  
  &  71.9  &  ILP  &  .439  &  .430  &  .432  &  .116  &  .111  &  .113  \\
  &    &  ILP+MC  &  .423  &  .417  &  .417  &  .101$^-$  &  .098$^-$  &  .099$^-$  \\
movie  &  76.4  &  ILP  &  .435  &  .424  &  .427  &  .091  &  .087  &  .088  \\
  &    &  ILP+MC  &  \bf{.436}  &  \bf{.427}  &  \bf{.429}  &  \bf{.106$^+$}  &  \bf{.100$^+$}  &  \bf{.102$^+$}  \\
  &  76.8  &  ILP  &  .435  &  .427  &  .428  &  .109  &  .105  &  .106  \\
  &    &  ILP+MC  &  .408  &  .402  &  .402  &  .100  &  .097  &  .098   \\
  \hline
  
  &  71.3  &  ILP  &  .467  &  .465  &  .465  &  .206  &  .201  &  .203  \\
  &    &  ILP+MC  &  .431  &  .447  &  .439  &  .163  &  .170  &  .166   \\
peer  &  77.1  &  ILP  &  .466  &  .469  &  .466  &  .199  &  .196  &  .197   \\
  &    &  ILP+MC  &  \bf{.491}  &  \bf{.496}  &  \bf{.492}  &  \bf{.261}  &  \bf{.262}  &  \bf{.260}  \\
  &  78.7  &  ILP  &  .488  &  .479  &  .482  &  .242  &  .229  &  .234  \\
  &    &  ILP+MC  &  .456  &  .466  &  .460  &  .204  &  .207  &  .205  \\
  \hline
%  &  12.6  &  ILP  &  .376  &  .380  &  .378  &  .092  &  .093  &  .092  &  .125  &  .128  &  .126 \\
%  &    &  ILP+MC  &  .348$^-$  &  .352$^-$  &  .349$^-$  &  .074$^-$  &  .075$^-$  &  .074$^-$  &  .112$^-$  &  .115$^-$  &  .113$^-$ \\
  &  13.9  &  ILP  &  .376  &  .380  &  .378  &  .092  &  .093  &  .092   \\
  &    &  ILP+MC  &  .349$^-$  &  .350$^-$  &  .349$^-$  &  .074$^-$  &  .074$^-$  &  .074$^-$  \\
DUC04  &  15.9  &  ILP  &  .377  &  .381  &  .379  &  .092  &  .093  &  .092   \\
  &    &  ILP+MC  &  .342$^-$  &  .351$^-$  &  .346$^-$  &  .072$^-$  &  .074$^-$  &  .072$^-$  \\
  &  16.5  &  ILP  &  .375  &  .379  &  .377  &  .093  &  .094  &  .094   \\
  &    &  ILP+MC  &  .349$^-$  &  .351$^-$  &  .349$^-$  &  .074$^-$  &  .075$^-$  &  .074$^-$   \\\hline
  \hline
\end{tabular}
\end{footnotesize}

